VDNA-PR: Using General Dataset Representations for Robust Sequential Visual Place Recognition

This paper adapts a general dataset representation technique to produce robust Visual Place Recognition (VPR) descriptors, crucial to enable real-world mobile robot localisation. Two parallel lines of work on VPR have shown, on one side, that general-purpose off-the-shelf feature representations can provide robustness to domain shifts, and, on the other, that fused information from sequences of images improves performance. In our recent work on measuring domain gaps between image datasets, we proposed a Visual Distribution of Neuron Activations (VDNA) representation to represent datasets of images. This representation can naturally handle image sequences and provides a general and granular feature representation derived from a general-purpose model. Moreover, our representation is based on tracking neuron activation values over the list of images to represent and is not limited to a particular neural network layer, therefore having access to high- and low-level concepts. This work shows how VDNAs can be used for VPR by learning a very lightweight and simple encoder to generate task-specific descriptors. Our experiments show that our representation can allow for better robustness than current solutions to serious domain shifts away from the training data distribution, such as to indoor environments and aerial imagery.

==> tabs/combined_urban_nonurban_results_flipped.tex <==
\begin{table*}[!h]
\centering
\caption{Performance comparison on benchmark environments with \textbf{non-urban environments} (left) and in \textbf{urban environments} (right).
Please refer to the baseline/ablation definitions in~\cref{sec:exp:baselines} for details of methods (row names).
}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccccccc|cccccccccccc} & \multicolumn{2}{c}{\textbf{Baidu Mall}} & \multicolumn{2}{c}{\textbf{Gardens Point}} & \multicolumn{2}{c}{\textbf{17 Places}} & \multicolumn{2}{c}{\textbf{VPAIR}} & \multicolumn{2}{c}{\textbf{MSLS}} & \multicolumn{2}{c}{\textbf{St Lucia}} & \multicolumn{2}{c}{\textbf{Pitts-30k}} & \multicolumn{2}{c}{\textbf{RobotCar 1}} & \multicolumn{2}{c}{\textbf{RobotCar 2}} & \multicolumn{2}{c}{\textbf{RobotCar 3}}\\
& R@1 & R@5 & R@1 & R@5 & R@1 & R@5 & R@1 & R@5 & R@1  & R@5  & R@1  & R@5  & R@1  & R@5  & R@1  & R@5  & R@1  & R@5   & R@1   & R@5 \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}  \cmidrule(lr){12-13}  
\ref{seqvlad}                     & 52.1 & 69.5 & 89.8 & 95.9 & 81.1 & 86.8 & 20.5 & 30.5  & \textbf{87.9} & \textbf{91.7} & \textbf{99.7} & \textbf{99.9} & 92.8 & 96.1 & 35.5 & 45.1 & 97.0 & 98.1  & 68.3  & 76.9 \\
\ref{seqvlad_frozen_encoder}    & 63.5 & 80.4 & \textbf{100.0}& \textbf{100.0}& \textbf{83.5} & \textbf{89.8} & 44.4 & 57.2 & 82.2 & 87.6 & 99.5 & \textbf{99.9} & \textbf{93.4} & \textbf{96.6} & \textbf{66.0} & \textbf{74.1} & \textbf{98.3} & \textbf{98.9}  & \textbf{93.3}  & \textbf{96.3} \\
\ref{vlad}                        & 50.9 & 73.4 & 97.4 & \textbf{100.0}& 81.7 & 87.7 & 20.7 & 34.5 & 44.7 & 57.2 & 62.6 & 76.8 & 76.7 & 89.3 & 33.0 & 51.4 & 86.1 & 95.1  & 58.0  & 77.1   \\
\ref{vdna_trained_linear_layer} & 37.1 & 63.8 & 88.3 & 95.4 & 78.7 & 88.6 & 24.8 & 41.7 & 74.1 & 84.0 & 92.1 & 95.3 & 81.2 & 93.2 & 34.7 & 49.9 & 92.2 & 96.8  & 69.8  & 86.2  \\
\ref{vdna_all_neurons}          & 49.7 & 72.8 & 99.0 & \textbf{100.0}& 80.2 & \textbf{89.8} & 40.4 & 50.4 & 38.9 & 46.0 & 79.2 & 86.1 & 81.7 & 88.7 & 8.6  & 19.6 & 91.0 & 94.5  & 51.9  & 72.4 \\
\ref{vdna_layer_12}             & 64.5 & \textbf{81.5} & \textbf{100.0}& \textbf{100.0}& 82.9 & \textbf{89.8} & 50.2 & 63.5 & 49.8 & 58.5 & 91.3 & 95.1 & 87.6 & 94.4 & 29.2 & 40.6 & 93.8 & 96.5  & 78.9  & 88.1  \\
\ref{vdna_layer_9_to_12}        & 66.0 & 81.2 & \textbf{100.0}& \textbf{100.0}& 82.3 & 89.2 & \textbf{51.3} & 63.2 & 45.4 & 52.6 & 86.1 & 91.7 & 85.4 & 92.0 & 30.6 & 42.5 & 94.6 & 97.3  & 78.5  & 88.4  \\
\ref{vdna_layer_10_to_12}        & \textbf{66.2} & 81.3 & 99.5 & \textbf{100.0}& 82.0 & 89.2 & 51.1 & 63.7 & 46.0 & 54.1 & 87.1 & 92.2 & 86.0 & 92.6 & 29.9 & 41.4 & 94.9 & 97.4  & 77.9  & 87.8  \\
\ref{vdna_layer_11_to_12}        & 65.4 & 81.4 & \textbf{100.0}& \textbf{100.0}& 82.9 & 89.5 & 51.0 & \textbf{64.3} & 46.7 & 54.5 & 88.6 & 93.6 & 86.2 & 92.9 & 28.3 & 40.9 & 93.7 & 96.7  & 78.3  & 87.9  \\
\end{tabular}
}
\label{tab:combined_urban_nonurban_results}
\end{table*}

==> tabs/nonurban_results.tex <==
\begin{table*}[!h]
\centering
\caption{Performance comparison on benchmark environments with \textbf{domain shifts}.}
\begin{tabular}{ccccccccc} & \multicolumn{2}{c}{\textbf{Baidu Mall}} & \multicolumn{2}{c}{\textbf{Gardens Point}} & \multicolumn{2}{c}{\textbf{17 Places}} & \multicolumn{2}{c}{\textbf{VPAIR}}\\
& R@1 & R@5 & R@1 & R@5 & R@1 & R@5 & R@1 & R@5  \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}  
SeqVLAD                     & 52.1 & 69.5 & 89.8 & 95.9 & 81.1 & 86.8 & 20.5 & 30.5   \\
SeqVLAD - frozen encoder    & 63.5 & 80.4 & \textbf{100.0}& \textbf{100.0}& \textbf{83.5} & \textbf{89.8} & 44.4 & 57.2 \\
VLAD                        & 50.9 & 73.4 & 97.4 & \textbf{100.0}& 81.7 & 87.7 & 20.7 & 34.5   \\
VDNA + trained linear layer & 37.1 & 63.8 & 88.3 & 95.4 & 78.7 & 88.6 & 24.8 & 41.7  \\
VDNA + all neurons          & 49.7 & 72.8 & 99.0 & \textbf{100.0}& 80.2 & \textbf{89.8} & 40.4 & 50.4 \\
VDNA + layer 12             & 64.5 & \textbf{81.5} & \textbf{100.0}& \textbf{100.0}& 82.9 & \textbf{89.8} & 50.2 & 63.5  \\
VDNA + layer 9 to 12        & 66.0 & 81.2 & \textbf{100.0}& \textbf{100.0}& 82.3 & 89.2 & \textbf{51.3} & 63.2  \\
VDNA + layer 10 to 12       & \textbf{66.2} & 81.3 & 99.5 & \textbf{100.0}& 82.0 & 89.2 & 51.1 & 63.7  \\
VDNA + layer 11 to 12       & 65.4 & 81.4 & \textbf{100.0}& \textbf{100.0}& 82.9 & 89.5 & 51.0 & \textbf{64.3}  \\
\end{tabular}
\label{tab:nonurban_results}
\end{table*}

==> tabs/urban_results.tex <==
\begin{table*}[!h]
\centering
\caption{Performance comparison on benchmark \textbf{urban} environments.}
\begin{tabular}{ccccccccccccc} & \multicolumn{2}{c}{\textbf{MSLS}} & \multicolumn{2}{c}{\textbf{St Lucia}} & \multicolumn{2}{c}{\textbf{Pitts-30k}} & \multicolumn{2}{c}{\textbf{RobotCar 1}} & \multicolumn{2}{c}{\textbf{RobotCar 2}} & \multicolumn{2}{c}{\textbf{RobotCar 3}}\\
& R@1  & R@5  & R@1  & R@5  & R@1  & R@5  & R@1  & R@5  & R@1  & R@5   & R@1   & R@5   \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}  \cmidrule(lr){12-13}
SeqVLAD                     & \textbf{87.9} & \textbf{91.7} & \textbf{99.7} & \textbf{99.9} & 92.8 & 96.1 & 35.5 & 45.1 & 97.0 & 98.1  & 68.3  & 76.9  \\
SeqVLAD - frozen encoder    & 82.2 & 87.6 & 99.5 & \textbf{99.9} & \textbf{93.4} & \textbf{96.6} & \textbf{66.0} & \textbf{74.1} & \textbf{98.3} & \textbf{98.9}  & \textbf{93.3}  & \textbf{96.3}  \\
VLAD                        & 44.7 & 57.2 & 62.6 & 76.8 & 76.7 & 89.3 & 33.0 & 51.4 & 86.1 & 95.1  & 58.0  & 77.1  \\
VDNA + trained linear layer & 76.1 & 84.0 & 92.1 & 95.3 & 81.2 & 93.2 & 34.7 & 49.9 & 92.2 & 96.8  & 69.8  & 86.2  \\
VDNA + all neurons          & 38.9 & 46.0 & 79.2 & 86.1 & 81.7 & 88.7 & 8.6  & 19.6 & 91.0 & 94.5  & 51.9  & 72.4  \\
VDNA + layer 12             & 49.8 & 58.5 & 91.3 & 95.1 & 87.6 & 94.4 & 29.2 & 40.6 & 93.8 & 96.5  & 78.9  & 88.1  \\
VDNA + layer 9 to 12        & 45.4 & 52.6 & 86.1 & 91.7 & 85.4 & 92.0 & 30.6 & 42.5 & 94.6 & 97.3  & 78.5  & 88.4  \\
VDNA + layer 10 to 12       & 46.0 & 54.1 & 87.1 & 92.2 & 86.0 & 92.6 & 29.9 & 41.4 & 94.9 & 97.4  & 77.9  & 87.8  \\
VDNA + layer 11 to 12       & 46.7 & 54.5 & 88.6 & 93.6 & 86.2 & 92.9 & 28.3 & 40.9 & 93.7 & 96.7  & 78.3  & 87.9  \\
\end{tabular}
\label{tab:urban_results}
\end{table*}
